Permutation-Invariant Graph Partitioning:How Graph Neural Networks Capture Structural Interactions?

Graph Neural Networks (GNNs) have paved the way for being a cornerstone in graph-related learning tasks. Yet, the ability of GNNs to capture structural interactions within graphs remains under-explored. In this work, we address this gap by drawing on the insight that permutation invariant graph partitioning enables a powerful way of exploring structural interactions. We establish theoretical connections between permutation invariant graph partitioning and graph isomorphism, and then propose Graph Partitioning Neural Networks (GPNNs), a novel architecture that efficiently enhances the expressive power of GNNs in learning structural interactions. We analyze how partitioning schemes and structural interactions contribute to GNN expressivity and their trade-offs with complexity. Empirically, we demonstrate that GPNNs outperform existing GNN models in capturing structural interactions across diverse graph benchmark tasks.

==> sections/checklist.tex <==
\clearpage
\section{Reproducibility Checklist}

\begin{itemize}
    \item This paper:
    \begin{itemize}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \hspace{1em} \textbf{(yes)}
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \hspace{1em} \textbf{(yes)}
        \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \hspace{1em} \textbf{(yes)}
        \item Does this paper make theoretical contributions? \hspace{1em} \textbf{(yes)}
    \end{itemize}

    If yes, please complete the list below.

    \begin{itemize}
        \item All assumptions and restrictions are stated clearly and formally \hspace{1em} \textbf{(yes)}
        \item All novel claims are stated formally (e.g., in theorem statements) \hspace{1em} \textbf{(yes)}
        \item Proofs of all novel claims are included \hspace{1em} \textbf{(yes)}
        \item Proof sketches or intuitions are given for complex and/or novel results \hspace{1em} \textbf{(yes)}
        \item Appropriate citations to theoretical tools used are given \hspace{1em} \textbf{(yes)}
        \item All theoretical claims are demonstrated empirically to hold \hspace{1em} \textbf{(partial)}
        \item All experimental code used to eliminate or disprove claims is included \hspace{1em} \textbf{(NA)}
    \end{itemize}

    \item Does this paper rely on one or more datasets? \hspace{1em} \textbf{(yes)}

    If yes, please complete the list below.

    \begin{itemize}
        \item A motivation is given for why the experiments are conducted on the selected datasets \hspace{1em} \textbf{(yes)}
        \item All novel datasets introduced in this paper are included in a data appendix \hspace{1em} \textbf{(NA)}
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes \hspace{1em} \textbf{(NA)}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations \hspace{1em} \textbf{(yes)}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available \hspace{1em} \textbf{(yes)}
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying \hspace{1em} \textbf{(NA)}
    \end{itemize}

    \item Does this paper include computational experiments? \hspace{1em} \textbf{(yes)}

    If yes, please complete the list below.

    \begin{itemize}
        \item Any code required for pre-processing data is included in the appendix \hspace{1em} \textbf{(NA)}
        \item All source code required for conducting and analyzing the experiments is included in a code appendix \hspace{1em} \textbf{(yes)}
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes \hspace{1em} \textbf{(yes)}
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \hspace{1em} \textbf{(yes)}
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results \hspace{1em} \textbf{(yes)}
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks \hspace{1em} \textbf{(yes)}
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics \hspace{1em} \textbf{(no)}
        \item This paper states the number of algorithm runs used to compute each reported result \hspace{1em} \textbf{(yes)}
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information \hspace{1em} \textbf{(yes)}
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank) \hspace{1em} \textbf{(no)}
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments \hspace{1em} \textbf{(no)}
        \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting \hspace{1em} \textbf{(yes)}
    \end{itemize}
\end{itemize}


==> sections/preliminaries.tex <==





\section{Preliminaries}

Let $G$ be a simple graph, and $V(G)$ and $E(G)$ refer to the set of vertices and the set of edges of $G$, respectively. % and $A\in \{0,1\}^{|V|\times|V|}$ is the adjacent matrix of $G$ where $A_{ij}=0$ denotes $(v_i,v_j)\notin E$ and $A_{ij}=1$ for $(v_i,v_j)\in E$. 
%\q{$X\in \mathbb{R}^{|V|\times m}$ is a feature matrix of $G$, where each vertex $v$ is associated with a feature vector $x_v\in \mathbb{R}^m$.}
Given $d\in \mathbb{N}$, for each $v\in V(G)$, the set of $d$-hop neighbouring vertices is denoted as $N_d(v) = \{u \in V(G) \mid (u,v)\in E(G), \delta(u,v)\leq d\}$, where $\delta(u,v)$ refers to the shortest-path distance between two vertices $u$ and $v$. When $d$ is equal to 1, we denote it as $N(v)$.
%Let $U\subseteq V$ be a vertex subset of a graph $G=(V,E)$. 
An induced subgraph of $G$ by $U\subseteq V(G)$ is the graph $G[U]$ whose vertex set is $U$ and edge set consists of the edges of $G$ that have endpoints in $U$, and we denote this as $G[U]\subseteq G$.
Two graphs $G_1$ and $G_2$ are \emph{isomorphic}, denoted as $G_1\simeq G_2$, if there exists a bijective mapping $g: V(G_1)\rightarrow V(G_2)$ such that $(v,u)\in E(G_1)$ iff $(g(v),g(u))\in E(G_2)$. A permutation $\pi$ of a graph $G$ is a bijection of $G$ onto itself such that $\pi(G)=(\pi(V(G)), \pi(E(G)))$, $\pi(V(G))=V(G)$, and $\pi(E(G))=\{(\pi(v),\pi(u)|(v,u)\in E(G)\}$. A function $f$ is \emph{permutation-invariant} iff $f(G) = f(\pi(G))$. 




==> sections/proposed-model.tex <==
\section{Proposed Method}

We propose a novel GNN that consists of two primary components: a) An \emph{inter-interaction} module to capture interactions within subgraphs b) An \emph{intra-interaction} module to capture interactions between different subgraphs.


Let $(G_1,\dots, G_k)$ be a sequence of disjoint subgraphs generated by $\{\mathcal{F}_{\varphi_i}\}_{i\in[1,k]}$ over $G$. For each vertex $v\in V$, inter-interaction module selects a subset of nodes from the the corresponding neighbourhood $N_{d1}(v)$ where $\forall u \in N_{d1}(v), \lambda(u) = \lambda(v)$. Suppose that $\gamma_v^{(0)}\in \mathbb{R}$ and $\gamma_v^{(0)}= \textsc{Deg}(v)$ for 
any $\{u,v\}\subseteq V(G)$,. For each vertex $v\in V(G)$, we embed its inter-interactions into a continuous space, represented by $\gamma_v^{(\ell+1)}$ as,
\begin{align}
\gamma_v^{(\ell+1)}= &\textsc{Upd}\left(\gamma_v^{(\ell)}, \textsc{Agg}\left(\{\!\!\{\gamma_u^{(\ell)}|u\in N^j_{d1}(v), \lambda(v)=j\}\!\!\}\right)\right)
\end{align}


%\begin{multline}
%\gamma_v^{(\ell+1)}= &\textsc{Upd}\left(\gamma_v^{(\ell)}, \textsc{Agg}\left(\{\!\!\{\gamma_u^{(\ell)}|u\in N^j_{d1}(v), \lambda(v)=j\}\!\!\}\right), &\textsc{Agg}\left(\{\!\!\{\gamma_u^{(\ell)}|u\in N_{d1}(v)\}\!\!\}\right)\right)
%\end{multline}

Then, the intra-interaction module partitions the corresponding neighbourhood $N_{d2}(v)$ for vertex $v \in V(G)$ into a set of neighbouring 
vertex subsets $\{N_{d2}^1(v),\dots, N_{d2}^k(v)\}$ where $N_{d2}^i(v)\subseteq V(G_{i})$, $\bigcup_{j\in[1,k]}N_{d2}^j(v)=N_{d2}(v)$, and 
$\bigwedge_{1\leq i\neq j\leq k} N_{d2}^i(v)\cap N_{d2}^j(v)=\emptyset$. 
 Based on the representations of inter-interactions among vertices, the representation $\Gamma_v$ of intra-interaction for vertex $v$ is defined as,
\begin{align}
 \Gamma_{v}=&\textsc{Agg}\Bigl(\{\!\!\{(\gamma_u^{(\ell+1)}, \alpha_{u,v})|u\in N_{d2}^1(v)\}\!\!\}, \dots, \nonumber\\& \hspace*{0.9cm}\{\!\!\{(\gamma_u^{(\ell+1)}, \alpha_{u,v})|u\in N_{d2}^k(v)\}\!\!\}\Bigr) 
\end{align}

 Note that $\alpha(u,v) \in \mathbb{R}$ denotes  features for intra-interaction edges.

The intra-interaction embedding $\gamma_v^{(\ell+1)}$ is then combined into the inter-interaction embedding $\Gamma_{v}$ to derive the final node embedding $h_{v}$. 
\begin{align}
h_v=&\textsc{Combine}\left(h_v^{gnn},\langle \gamma_v^{(\ell+1)}, \Gamma_{v}\rangle\right).
%h_v=&\textsc{Cmb}\left(\gamma_v^{(\ell+1)}, \Gamma_{v}\right).
\end{align}

This will be followed by a graph readout step to generate the graph embedding, denoted by $h_G$. Furthermore, we combine global structural information related to graph decomposition, denoted by $c_G$, into the final embedding to strengthen the representation.
\begin{align}
%    h_G=&\textsc{Readout}\Bigl( \textsc{Agg}\left(\{\!\!\{h_v| v\in V(G)\}\!\!\}\right), c_G\Bigr).
    h_G=&\textsc{Readout}\Bigl( \{\!\!\{h_v| v\in V(G)\}\!\!\}, c_G\Bigr).
\end{align}

==> sections/results-and-discussion.tex <==
\section{Results and Discussion}
In this section we discuss the results of our experiments.
\subsection{Graph Classification}

\paragraph{TU Datasets} Table \ref{Tab:graph-classification-baselines} reports the results on small-scale datasets in graph classification task. % under the settings given by \citet{xu2018powerful} and \citet{feng2022powerful}. 
We can see that both GPNN$^{\star}$ and  GPNN$^{\dagger}$ models surpass existing baselines in both evaluation settings. GPNN significantly outperforms state-of-the-art methods under Setting 2 on datasets like PROTEINS and BZR.  The performance of GPNN$^{\star}$ also shows that interactions from intra-edges may carry new and useful information, contributing to graph classification on real-world datasets. As intra-edges are usually a small subset of all edges in a graph, GPNN$^{\star}$ enables an efficient yet expressive solution for many graph classification tasks.

\begin{table*}
\centering 
\scalebox{1}{\begin{tabular}{l| c c c c c c }
\specialrule{.1em}{.05em}{.05em} 
Experimental Setups & Methods & MUTAG & PTC-MR & PROTEINS & BZR & COX2  \\ [0.5ex] 
\hline
\multirow{6}{*}{\shortstack{Setting 1\\ \citep{xu2018powerful}}} & {GIN} & {89.4 ± 5.6} & {64.6 ± 7.0} & {75.9 ± 2.8}  & {85.6 ± 2.0} & {82.44 ± 3.0} \\ 
%\q{DGCNN} & {85.8 ± 1.7} & {58.6 ± 2.5} & {75.5 ± 0.9} & {-} &{-} \\ 
 & {GraphSNN} & {91.24 ± 2.5} & \textcolor{darkblue}{\textbf{66.96 ± 3.5}} & {76.51 ± 2.5}  & \textcolor{darkblue}{\textbf{88.69 ± 3.2}} & {82.86 
 ± 3.1} \\ 
 & {GIN-AK+} & {91.30 ± 7.0} & \textbf{{68.20 ± 5.6}} &\textcolor{darkblue}{\textbf{77.10 ± 5.7}} & {-} & {-} \\ 
 & {KP-GIN} & \textcolor{darkblue}{\textbf{92.2 ± 6.5}} & {66.8 ± 6.8} & {75.8 ± 4.6

} & {-} & {-} \\ 
%\q{GSN} & {92.2 ± 7.5} & {68.2 ± 7.2} & {76.6 ± 5.0}  & {-} & {-} \\ 
\cline{2-7} %inserts single line
 & {GPNN$^{\star}$} & {91.02 ± 7.1} & {66.20 ± 11.2} & \textbf{77.18 ± 4.6}  & {88.60 ± 4.6} & \textcolor{darkblue}{\textbf{82.88 ± 4.6}} \\ 
 & {GPNN$^{\diamond}$} & \textbf{{92.60 ± 4.8}} & {65.95 ± 8.5} & {76.82 ± 3.9}  & \textbf{{89.12 ± 2.3}} &  \textbf{{83.09 ± 3.1}} \\ 
\hline\hline
\multirow{6}{*}{\shortstack{Setting 2\\ \citep{feng2022powerful}}} & {GIN} & {92.8 ± 5.9} & {65.6 ± 6.5} & {78.8 ± 4.1}  & {91.05 ± 3.4} & {88.87 ± 2.3} \\ 
 & {GraphSNN} & {94.70 ± 1.9} & {70.58 ± 3.1} & {78.42 ± 2.7}  & {91.12 ± 3.0} & {86.28 ± 3.3} \\ 
 & {GIN-AK+} & {95.0 ± 6.1} & {74.1 ± 5.9} & {78.9 ± 5.4} & {-} & {-} \\ 
 & {KP-GIN} & {95.6 ± 4.4} & {76.2 ± 4.5} & {79.5 ± 4.4} & {-} & {-} \\ 
\cline{2-7} %inserts single line
 & {GPNN$^{\star}$} & \textbf{{97.89 ± 2.6}} & \textcolor{darkblue}{\textbf{78.17 ± 6.2}} & \textcolor{darkblue}{\textbf{81.40 ± 3.5}}  & \textbf{{94.05 ± 2.6}} & \textcolor{darkblue}{\textbf{89.09 ± 3.3}} \\ 
 & {GPNN$^{\diamond}$} & \textcolor{darkblue}{\textbf{97.37 ± 4.9}} & \textbf{{79.61 ± 7.3}} & \textbf{85.53 ± 6.2}  & \textcolor{darkblue}{\textbf{91.84 ± 1.6}} & \textbf{{89.72 ± 2.3}} \\ 
\hline %inserts single line
\end{tabular}}
\caption{Graph classification accuracy (\%) ± standard deviation (\%) for TU datasets. %under setting 1 \citep{xu2018powerful} and setting 2 \citep{feng2022powerful}. 
Under each setting, best results are highlighted in \textbf{black} and second best results are highlighted in \textcolor{darkblue}{\textbf{blue}}. The results of baselines for MUTAG, PTC\_MR and PROTEINS datasets are taken from \citet{feng2022powerful}. The results of BZR and COX2 datasets are taken from \citet{wijesinghe2022new}, and \citet{you2021identity}. \q{For any baseline that is not reported in these papers, we use all settings the same as GPNN and report the results.(?)}
}
\label{Tab:graph-classification-baselines} \vspace*{-0.4cm}
\end{table*}

\paragraph{OGB Datasets} 
Table~\ref{Tab:ogb-classification-baselines}  reports the results on large-scale molecular datasets. Both variants of our model show comparable performance with other baselines. Additional structural information captured by GPNN adds more expressive power to the model that surpasses the performance of GIN which is known to have equivalent expressive power of 1-WL. Some baselines like CIN and GSN embed explicit structural information like cycle counts into node features in the learning process, which are known to have high correlations with molecular classes and features. In order to maintain generalizability, GPNN does not process any such hand selected domain-specific structural information.

\begin{table}[H]
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc} 
\toprule
{Methods}& \begin{tabular}{c}ogbg-\\molhiv\end{tabular} & \begin{tabular}{c}ogbg-\\moltoxcast\end{tabular} & \begin{tabular}{c}ogbg-\\moltox21\end{tabular}  \\ 
\midrule
{GIN} & { 75.58 ± 1.40} & {63.41 ± 0.74} & {74.91 ± 0.51} \\
{GraphSNN} & {78.51 ± 1.70} & \textbf{{65.40 ± 0.71}} & {75.45 ± 1.10} \\
%\q{k-Recon. GNN} & {-} & {65.36 ± 0.49} & {76.84 ± 0.62} \\
{PNA} & \textcolor{darkblue}{\textbf{79.05 ± 1.30}} & {-} & {-} \\
%{Deep LRP} & {77.19 ± 1.40} & {-} & {-} \\
\midrule
{GSN$^{\#}$} & {77.99 ± 1.00} & {-} & {-} \\
{CIN$^{\#}$} & \textbf{{80.94 ± 0.57}} & {-} & {-} \\
\midrule

{GPNN$^{\star}$} & {78.12 ± 1.91} & \textcolor{darkblue}{\textbf{64.70 ± 0.44}} & \textbf{{76.13 ± 0.68}} \\
\q{GPNN$^{\diamond}$} & {77.70 ± 2.23} & {64.48 ± 0.45} & \textcolor{darkblue}{\textbf{75.98 ± 0.39}} \\
\bottomrule
\end{tabular}}
\caption{Graph classification ROC (\%) ± standard deviation (\%) for OGB datasets. Best results are highlighted in \textbf{black} and second best results are highlighted in \textcolor{darkblue}{\textbf{blue}}. Results of GIN and GraphSNN are taken from \citet{wijesinghe2022new}. For other baseline results, we refer to \citet{bodnar2021weisfeiler}. \q{The  methods marked by \#
are based on pre-selected  domain-specific structural information. (discuss)}\q{Asela: depending on your results on GPNN$^{\diamond}$ under degree, maybe GPNN$^{\diamond}$ can be replaced by GPNN$^{\star}$ under degree - let's discuss this after you obtain the complete results.}}
\label{Tab:ogb-classification-baselines}
\end{table}
\smallskip
\subsection{Ablation Studies} We perform an ablation study to understand how partitioning schemes may affect the performance of GPNN. We denote GPNN variants with a trivial graph partitioning scheme as $\lambda_{\bot}$-GPNN$^{\delta}$ and with the graph partitioning scheme $\Phi_{core\text{-}degree}$ as $\lambda_{core\text{-}degree}$-GPNN$^{\delta}$, respectively. We use two datasets from TU repository \citep{morris2020tudataset} for the evaluation alongside the setup introduced by \citet{feng2022powerful}. Results are reported in Table \ref{Tab:ablation}.

\begin{table}[]
\centering
\begin{tabular}{ccc} 
\toprule
{Methods}& {DHFR} & {PTC\_FM}  \\ 
\midrule
{GIN\hspace{0.45cm}} & {80.04 ± 4.9} & {70.50 ± 4.7}  \\
\midrule
{$\lambda_{\bot}$-GPNN$^{\star}$} & {80.03 ± 4.0} & {70.78 ± 4.1}  \\
{$\lambda_{\bot}$-GPNN$^{\diamond}$} & {80.30 ± 3.0 } & {71.34 ± 4.6} \\
{$\lambda_{\bot}$-GPNN$^{\dagger}$} & {78.97 ± 4.0} & {73.15 ± 3.7} \\
\midrule
{$\lambda_{core\text{-}degree}$-GPNN$^{\star}$} & {82.01 ± 2.3} & {73.92 ± 6.0}  \\
{$\lambda_{core\text{-}degree}$-GPNN$^{\diamond}$} & {82.15 ± 2.9} & {73.92 ± 4.9} \\
{$\lambda_{core\text{-}degree}$-GPNN$^{\dagger}$} & {80.16 ± 2.6} & {74.50 ± 5.8} \\
\bottomrule
\end{tabular}
\caption{Ablation study accuracy (\%) ± standard deviation (\%) for DHFR and PTC\_FM datasets. \q{(we need to discuss whether these twp datasets can be replaced by the OGB datasets.)}} 
\label{Tab:ablation}
\end{table}

From the results, we can see that GPNNs using $\Phi_{core\text{-}degree}$ perform better than ones using a trivial partitioning scheme. $\lambda_{\bot}$-GPNN$^{\star}$ has similar results to GIN, which provides empirical evidence about its expressive power being aligned with Theorem \ref{thm-triviallambda}. Further, when the partitioning scheme is $\Phi_{core\text{-}degree}$, GPNNs show considerable improvements over GIN. This empirically validates Theorem \ref{thm-nontriviallambda}. Furthermore, $\lambda_{\bot}$-GPNN$^{\dagger}$ and $\lambda_{core\text{-}degree}$-GPNN$^{\dagger}$ achieve the highest improvement for PTC\_FM dataset, which is consistent with their theoretical expressive powers. However, this does not hold true for DHFR dataset as GPNN$^{\dagger}$ variants show lower performance. We believe that this happens due to the higher computational complexity and large learnable parameter space introduced by GPNN$^{\dagger}$ variants that could hamper the training process on that dataset.



==> sections/theoretical-analysis.tex <==
\section{Theoretical Analysis}

\subsection{Expressivity Analysis}

\begin{lemma} Core-decomposition coloring is strictly less expressive than 1-WL
\end{lemma}


\begin{lemma} Onion-decomposition coloring is strictly less expressive than 1-WL, but strictly more expressive than core-decomposition coloring.
\end{lemma}

\begin{theorem} ???GNN with injective \textsc{Upd}, \textsc{Agg}, and \textsc{Cmb} functions, is strictly more expressive as 1-WL.
\end{theorem}



